Generating Efficient DNN-Ensembles with Evolutionary Computation

In this work, we leverage ensemble learning as a tool for the creation of faster, smaller, and more accurate deep learning models. We demonstrate that we can jointly optimize for accuracy, inference time, and the number of parameters by combining DNN classifiers. To achieve this, we combine multiple ensemble strategies: bagging, boosting, and an ordered chain of classifiers. To reduce the number of DNN ensemble evaluations during the search, we propose EARN, an evolutionary approach that optimizes the ensemble according to three objectives regarding the constraints specified by the user. We run EARN on 10 image classification datasets with an initial pool of 32 state-of-the-art DCNN on both CPU and GPU platforms, and we generate models with speedups up to $7.60\times$, reductions of parameters by $10\times$, or increases in accuracy up to $6.01\%$ regarding the best DNN in the pool. In addition, our method generates models that are $5.6\times$ faster than the state-of-the-art methods for automatic model generation.

==> tables/exp1_cpu.tex <==
\begin{table*} \centering
\caption{CPU}
\label{table:earn_bigtable}
\small
    \begin{tabular}{|l||c|c|c||c|c|c||c|c|c|} \hline
    \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c|}{\textbf{Solution a}} & \multicolumn{3}{c|}{\textbf{Solution b}} & \multicolumn{3}{c|}{\textbf{Solution c}}\\ 
    \cline{2-10} &  Acc. & Sp. & Size &  Acc. & Sp. & Size &  Acc. & Sp. & Size\\ \hline\hline
    cifar10 
      & +0,56\% & 0,62$\times$ & 2,95$\times$ & +0,09\% & 3,66$\times$ & 1,47 $\times$ & +0,06\% & 1,65$\times$ & 0,35$\times$ \\
     \hline
    cifar100
     & +2,59\% & 0,38$\times$ & 3,13$\times$ & +0,18\% & 2,36$\times$ & 1,35$\times$ & +0,65\% & 1,28$\times$ & 0,31$\times$\\
     \hline
    svhn
     & +0,07\% & 0,70$\times$ & 1,10$\times$ & +0,06\% & 1,80$\times$ & 0,90$\times$ & +0,02\% & 0,63$\times$ & 0,30$\times$\\
     \hline
    stl10
     & +4,02\% & 0,40$\times$ & 7,80$\times$ & +0,17\% & 3,15$\times$ & 3,00$\times$ & +0,16\% & 0,71$\times$ & 0,94$\times$\\
     \hline
    mnist
     & +0,00\% & 1,00$\times$ & 1,00$\times$ & +0,00\% & 1,00$\times$ & 1,00$\times$ & +0,00\% & 1,00$\times$ & 1,00$\times$\\
     \hline
    gtsrb 
    & +0,41\% & 0,87$\times$ & 5,46$\times$ & +0,08\% & 3,15$\times$ & 2,98$\times$ & +0,01\% & 1,03$\times$ & 0,90$\times$\\
     \hline
    food101
    & +4,30\% & 0,34$\times$ & 3,40$\times$ & +0,19\% & 2,11$\times$ & 0,60$\times$ & +0,30\% & 1,46$\times$ & 0,28$\times$\\
     \hline
    flowers102
    & +7,30\% & 0,10$\times$ & 3,75$\times$ & +0,00\% & 1,00$\times$ & 1,00$\times$ & +2,10\% & 0,30$\times$ & 0,13$\times$\\
     \hline
    fashion
    & +0,35\% & 0,31$\times$ & 2,48$\times$ & +0,07\% & 1,48$\times$ & 0,97$\times$ & +0,04\% & 0,64$\times$ & 0,22$\times$\\
     \hline
    caltech256
    & +5,85\% & 0,59$\times$ & 1,65$\times$ & +0,19\% & 4,07$\times$ & 0,89$\times$ & +0,08\% & 2,46$\times$ & 0,14$\times$\\
     \hline
     \hline
     \textbf{Average} & +2,55\% & 0,53$\times$ & 3,27$\times$ & +0,10\% & 2,38$\times$ & 1,42$\times$ & +0,34\% & 1,12$\times$ & 0,45$\times$\\
     \hline
    \end{tabular}
\end{table*}

==> tables/exp1_gpu.tex <==
\begin{table*}[t] 
\centering
\caption{GPU}
\label{table:earn_bigtable}
\small
    \begin{tabular}{|l||c|c|c||c|c|c||c|c|c|} \hline
    \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c|}{\textbf{Solution a}} & \multicolumn{3}{c|}{\textbf{Solution b}} & \multicolumn{3}{c|}{\textbf{Solution c}}\\ 
    \cline{2-10} &  Acc. & Sp. & Size &  Acc. & Sp. & Size &  Acc. & Sp. & Size\\ \hline\hline
    cifar10 
      & +0,56\% & 0,62$\times$ & 2,95$\times$ & +0,09\% & 3,66$\times$ & 1,47 $\times$ & +0,06\% & 1,65$\times$ & 0,35$\times$ \\
     \hline
    cifar100
     & +2,59\% & 0,38$\times$ & 3,13$\times$ & +0,18\% & 2,36$\times$ & 1,35$\times$ & +0,65\% & 1,28$\times$ & 0,31$\times$\\
     \hline
    svhn
     & +0,07\% & 0,70$\times$ & 1,10$\times$ & +0,06\% & 1,80$\times$ & 0,90$\times$ & +0,02\% & 0,63$\times$ & 0,30$\times$\\
     \hline
    stl10
     & +4,02\% & 0,40$\times$ & 7,80$\times$ & +0,17\% & 3,15$\times$ & 3,00$\times$ & +0,16\% & 0,71$\times$ & 0,94$\times$\\
     \hline
    mnist
     & +0,00\% & 1,00$\times$ & 1,00$\times$ & +0,00\% & 1,00$\times$ & 1,00$\times$ & +0,00\% & 1,00$\times$ & 1,00$\times$\\
     \hline
    gtsrb 
    & +0,41\% & 0,87$\times$ & 5,46$\times$ & +0,08\% & 3,15$\times$ & 2,98$\times$ & +0,01\% & 1,03$\times$ & 0,90$\times$\\
     \hline
    food101
    & +4,30\% & 0,34$\times$ & 3,40$\times$ & +0,19\% & 2,11$\times$ & 0,60$\times$ & +0,30\% & 1,46$\times$ & 0,28$\times$\\
     \hline
    flowers102
    & +7,30\% & 0,10$\times$ & 3,75$\times$ & +0,00\% & 1,00$\times$ & 1,00$\times$ & +2,10\% & 0,30$\times$ & 0,13$\times$\\
     \hline
    fashion
    & +0,35\% & 0,31$\times$ & 2,48$\times$ & +0,07\% & 1,48$\times$ & 0,97$\times$ & +0,04\% & 0,64$\times$ & 0,22$\times$\\
     \hline
    caltech256
    & +5,85\% & 0,59$\times$ & 1,65$\times$ & +0,19\% & 4,07$\times$ & 0,89$\times$ & +0,08\% & 2,46$\times$ & 0,14$\times$\\
     \hline
     \hline
     \textbf{Average} & +2,55\% & 0,53$\times$ & 3,27$\times$ & +0,10\% & 2,38$\times$ & 1,42$\times$ & +0,34\% & 1,12$\times$ & 0,45$\times$\\
     \hline
    \end{tabular}
\end{table*}
